Fourier Series in Fractional Dimensional Space

In this paper, a Fourier series in fractional dimensional space is introduced for an arbitrarily periodic function $f(t;\alpha)$. We call it fractional Fourier series of the order $\alpha$. Extending the basis functions of the linear space into fractional one, by rotation transformation, we define a real and complex Fourier series and obtain their coefficients. It is also shown that the fractional derivative of a periodic function can be realized through (fractional) Fourier series with modified coefficients.

==> sn-sample-bib.tex <==
\begin{thebibliography}
%{99}

\bibitem{HA} M.A. Hammad and R.R. Khalil,"Fractional Fourier Series with Applications", Amer.J.Comput. Appl. Math., 4 (6), 187-191, 2014.

\bibitem{HM} M.-S. Hu, R. P. Agarwal, and X.-J. Yang, “Local fractional Fourier series with Application to Wave Equation in Fractal Vibrating String,” Abs. Appl. Analysis, 2012, Article ID 567401, 15 pages, 2012.

\bibitem{JG1} G. Jumarie, "Fourier’s transform of fractional order via Mittag-Leffler function and modified Riemann-Liouville derivative," J. Appl. Math. Informatics, 26 (5–6), 1101-1121, 2008.

\bibitem {MP}  P. R. Massopust and Ahmed I. Zayed. "On the Invalidity of Fourier series Expansions of Fractional Order." Fract. Calc. and Appl. Analysis, 18 (6),1507-1517, 2015.

\bibitem {OAV} A.V. Oppenheim, and A.S. Willsky, Signals and Systems, Prentice Hall, p.198, 1997 

\bibitem{PS} S.C. Pei, M.H. Yeh, and T.L. Luo, "Fractional Fourier Series Expansion for
Finite Signals and Dual Extension to Discrete-Time Fractional Fourier Transform", IEEE Trans.  Sig. Process. 47 (10), 2883-2888, 1999.

\bibitem{SH} H. M. Srivastava, A. K. Golmankhaneh, D. Baleanu, and X.-J.Yang, “Local Fractional Sumudu Transform with Application to IVPs on Cantor Sets,” Abs. and Appl. Analysis, vol. 2014, Article ID 620529, 7 pages, 2014.

\bibitem{WS} S.-Q. Wang, Y.-J. Yang, and H. K. Jassim, “Local Fractional
Function Decomposition Method for Solving Inhomogeneous Wave Equations with Local Fractional Derivative,” Abs. and Appl. Analysis, 2014, Article ID 176395, 7 pages, 2014.

\bibitem{YY} Y.J. Yang and S.Q. Wang "Local Fractional Fourier Series Method for Solving Nonlinear Equations with Local Fractional Operators", Math. Prob. Eng. 2015, Article ID: 481905, 9 pages, 2015. 

\bibitem{YC} C.Yu, "Fractional Fourier Series and its Applications", J. Physics: conference series, 1976, 2021.


\end{thebibliography}


